Apertus 1.5: From Open Text Models to Open Multimodal Reasoners

Language models are becoming infrastructure, and infrastructure built in the open, by public institutions, on documented data, is the alternative to dependence on a few providers; Apertus shows this is viable at scale. Apertus 1.5 extends the fully open Apertus family from text to multimodal reasoning. Continued pretraining of the Apertus 1.0 models, on 4T additional tokens for the 8B and 2T for the 70B, adds image and audio understanding and extends the context window fourfold to 262,144 tokens; multimodality enters through the tokenizer, the language-model head remains restricted to text, and the architecture is unchanged. Supervised finetuning, long-context finetuning, reinforcement learning with verifiable rewards, and preference alignment complete the released models. Thinking is a flag of the chat template rather than a separate model, and lifts mathematical reasoning by up to 20 points on the 8B model. The released models improve over their predecessors on nearly every benchmark; among fully open models of its class, the 8B leads on knowledge, instruction following, and cultural benchmarks, and its instruction following surpasses all compared models, including open-weight ones. On image and audio understanding, a first for the family, the models are competitive with fully open multimodal models, strongest on document understanding and long-form and lower-resource speech recognition, while specialized vision and audio models remain ahead on perception and transcription of English and other high-resource languages. As in Apertus 1.0, we train only on openly available data, respect crawler opt-outs retroactively, and exclude restrictively licensed material. We release the model weights, data preparation and training recipes, and evaluation suites under permissive licenses; openness extends to values, with the Apertus charter guiding alignment stages published alongside the models.

==> cover/authors.tex <==
% !TEX root = ../main.tex
\makeatletter
\newcounter{affcounter}
\gdef\aff@list{}
\newcommand{\affiliation}[2]{%
  \stepcounter{affcounter}%
  \expandafter\xdef\csname aff@num@#1\endcsname{\arabic{affcounter}}%
  \ifx\aff@list\@empty\else\g@addto@macro\aff@list{, }\fi
  \begingroup\edef\aff@tmp{\endgroup
    \noexpand\g@addto@macro\noexpand\aff@list{\noexpand\textsuperscript{\arabic{affcounter}}}}\aff@tmp
  \g@addto@macro\aff@list{#2}}
\newcommand{\aff@marks}[1]{{\def\aff@sep{}\@for\aff@k:=#1\do{\aff@sep\csname aff@num@\aff@k\endcsname\def\aff@sep{,}}}}
\newcommand{\au}[2]{#1\textsuperscript{\aff@marks{#2}}}
\newcommand{\cau}[2]{\textbf{#1}\textsuperscript{\aff@marks{#2}}}
\newcommand{\afflist}{\aff@list}

\def\@maketitle{\vbox{\hsize\textwidth
  {\LARGE\sc \@title\par}
  \vskip 0.8em
  \begingroup\parindent\z@\raggedright\baselineskip=12.5pt \lineskiplimit=-\maxdimen\relax
  \ificlrfinal\@author\else\bfseries Anonymous authors\par Paper under double-blind review\fi\par
  \endgroup
  \vskip 0.15in minus 0.05in}}
\makeatother

\affiliation{ethz}{ETH~Zurich}
\affiliation{epfl}{EPFL}
\affiliation{hevs}{HES\mbox{-}SO~Valais\mbox{-}Wallis}
\affiliation{fhnw}{FHNW}
\affiliation{sdsc}{SDSC}
\affiliation{cscs}{CSCS}
\affiliation{uzh}{University~of~Zurich}
\affiliation{bern}{University~of~Bern}

\author{%
\textbf{Project \apertus{}}\thanks{In each contribution level, team members are listed in (reverse) alphabetical order by first or last name. Contributions are described in more detail in \autoref{app:contributions}.}\\[0.6em]
\teamrow{Core Team}{\au{Yixuan~Xu}{ethz}, \au{Yassine~Turki}{epfl}, \au{Vinko~Sabolčec}{epfl}, \au{Valentina~Pyatkin}{ethz}, \au{Tommy~Chu}{epfl}, \au{Sven~Najem\mbox{-}Meyer}{epfl}, \au{Sean~F.~Carroll}{epfl}, \au{Robert~Smith}{ethz}, \au{Raphael~Kreft}{ethz}, \au{Oscar~Alessandro~Tazza}{ethz}, \au{Oleg~Lavrovsky}{epfl}, \au{Nicola~Irmiger}{ethz}, \au{Matteo~Santelmo}{epfl}, \au{Marian~Schneider}{ethz}, \au{Juan~García~Giraldo}{epfl}, \au{Hanna~Yukhymenko}{ethz}, \au{Eduard~Ďurech}{ethz}, \au{Davit~Melikidze}{ethz}, \au{Dani~Tamayo}{epfl}, \au{Bettina~Messmer}{epfl}, \au{Aryan~Ahadinia}{epfl}, \au{Anunay~Yadav}{epfl}, \au{Allen~Huang}{epfl}}
\teamrow{Contributors}{\au{Ahmad~Fraij}{ethz}, \au{Alessandro~Bombarda}{epfl}, \au{Alex~Padula}{ethz}, \au{Alexander~Hägele}{epfl}, \au{Alexander~Sternfeld}{hevs}, \au{Anna~Hedström}{ethz}, \au{Anna~Kosovskaia}{ethz}, \au{Arthur~Wuhrmann}{epfl}, \au{Arundhati~Balasubramaniam}{ethz}, \au{Badr~Al~Mahouri}{epfl}, \au{Barna~Pasztor}{ethz}, \au{Bartosz~Szostakiewicz}{ethz}, \au{Bich~Ngoc~Doan}{epfl}, \au{Bryan~Schmid}{fhnw}, \au{Burak~Sezen}{ethz}, \au{Camille~Challier}{epfl}, \au{Clément~Charmillot}{epfl}, \au{Dana~Shayakhmetova}{epfl}, \au{Daniel~Perruchoud}{fhnw}, \au{David~Brüggemann}{sdsc}, \au{David~Isztl}{cscs}, \au{Elia~Palme}{cscs}, \au{Emma~Anastassova}{epfl}, \au{Fabian~Bösch}{cscs}, \au{Faruk~Zahiragić}{epfl}, \au{Fawzi~Roberto~Mohamed}{cscs}, \au{Fiona~Panicali}{fhnw}, \au{Florian~Kolly}{epfl}, \au{Flynn~Guerra}{fhnw}, \au{Francesco~Monti}{epfl}, \au{Frederike~Lübeck}{ethz}, \au{Gennaro~Oliva}{cscs}, \au{Haofeng~Yang}{ethz}, \au{Haoliang~Shang}{ethz}, \au{Helen~El~Khoury}{epfl}, \au{Henrique~Mendonça}{cscs}, \au{Jannis~Vamvas}{uzh}, \au{Jérome~Landolt}{fhnw}, \au{Jessica~Lam}{ethz}, \au{Jingchun~Xiao}{ethz}, \au{Jonathan~Coles}{cscs}, \au{Joshua~Oyebanji}{epfl}, \au{Khanh~Nguyen}{epfl}, \au{Konstantinos~Pitas}{ethz}, \au{Lasse~B.~Strand}{ethz}, \au{Li~Mi}{ethz}, \au{Loïc~Deslarzes}{epfl}, \au{Lorenzo~Baggi}{ethz}, \au{Lorenzo~Noci}{ethz}, \au{Luca~Baumann}{ethz}, \au{Luca~Sartori}{ethz}, \au{Lukas~Drescher}{cscs}, \au{Marco~De~Negri}{ethz}, \au{Marco~Passerini}{cscs}, \au{Mark~Klein}{cscs}, \au{Marko~Stojanovic}{epfl}, \au{Martin~Majsec}{epfl}, \au{Matin~Ansaripour}{epfl}, \au{Mattea~Busato}{epfl}, \au{Mauro~Pellonara}{epfl}, \au{Max~Neuwinger}{ethz}, \au{Michael~Graber}{fhnw}, \au{Michal~Tešnar}{ethz}, \au{Michelle~Wastl}{uzh}, \au{Miguel~Gila}{cscs}, \au{Mikolaj~Boronski}{epfl}, \au{Morgane~Magnin}{epfl}, \au{Moritz~Reihs}{ethz}, \au{Mukhammadali~Sayfiddinov}{ethz}, \au{Nathan~Ranchin}{ethz,epfl}, \au{Nicolas~Cuveillier}{epfl}, \au{Oscar~Wohlfahrt}{epfl}, \au{Qianqian~Zou}{sdsc}, \au{Rada~Kamysheva}{ethz}, \au{Rita~Sevastjanova}{ethz}, \au{Roman~Machacek}{bern}, \au{Sebastian~Keller}{cscs}, \au{Simon~Matrenok}{epfl}, \au{Simon~Pierre}{epfl}, \au{Stefano~Schuppli}{cscs}, \au{Suei\mbox{-}Wen~Chen}{ethz}, \au{Szabina~Horváth\mbox{-}Mikulas}{epfl}, \au{Taliesin~Perez}{epfl}, \au{Thilo~Spinner}{ethz}, \au{Thomas~Kleine~Buening}{ethz}, \au{Tim~Robinson}{cscs}, \au{Tymoteusz~Kwiecinski}{ethz}, \au{Vilém~Zouhar}{ethz}, \au{Vinzenz~Thoma}{ethz}, \au{Xiaozhe~Yao}{ethz}, \au{Yannick~Metz}{ethz}, \au{Yuhei~Fukuhara}{epfl}, \au{Yusif~Askari}{epfl}, \au{Zixuan~Chen}{ethz}}
\teamrow{Advisors}{\au{Alexander~Ilic}{ethz}, \au{Ana~Klimovic}{ethz}, \au{Andreas~Krause}{ethz}, \au{Andrei~Kucharavy}{hevs}, \au{Elliott~Ash}{ethz}, \au{Joost~VandeVondele}{cscs}, \au{Martin~Rajman}{epfl}, \au{Mennatallah~El\mbox{-}Assady}{ethz}, \au{Thomas~Schulthess}{cscs}, \au{Timo~Kehrer}{bern}, \au{Torsten~Hoefler}{ethz}}
\teamrow{Leads}{\au{Antoine~Bosselut}{epfl}, \au{Martin~Jaggi}{epfl}, \au{Imanol~Schlag}{ethz}}
\affiliationsrow
}


==> figs/post_training/rl_ablation_benchmarks_data.tex <==
\newcommand{\RLBenchMathFiveHundred}{%
  \addplot[rl text,rl line,forget plot] coordinates {(0,58.4) (50,66.6) (100,72) (150,74.4) (200,71.8)};
  \addplot[rl mm,rl line,forget plot] coordinates {(0,59.4) (50,64) (100,70.2) (150,76.4) (200,76.4)};
  \addplot[rl prod,rl line,forget plot] coordinates {(0,79.8) (50,80.4) (100,81.2) (150,84.6) (200,81.6)};
}
\newcommand{\RLBenchAimeTwentyFive}{%
  \addplot[rl text,rl line,forget plot] coordinates {(0,7.604) (50,11.04) (100,11.46) (150,12.19) (200,11.46)};
  \addplot[rl mm,rl line,forget plot] coordinates {(0,11.67) (50,15) (100,16.04) (150,15.62) (200,18.44)};
  \addplot[rl prod,rl line,forget plot] coordinates {(0,21.77) (50,19.9) (100,21.04) (150,22.08) (200,22.6)};
}
\newcommand{\RLBenchAimeTwentySix}{%
  \addplot[rl text,rl line,forget plot] coordinates {(0,4.741) (50,4.957) (100,5.603) (150,5.711) (200,5.711)};
  \addplot[rl mm,rl line,forget plot] coordinates {(0,5.819) (50,7.328) (100,8.621) (150,10.13) (200,9.806)};
  \addplot[rl prod,rl line,forget plot] coordinates {(0,12.61) (50,13.25) (100,13.58) (150,16.16) (200,14.33)};
}
\newcommand{\RLBenchBBH}{%
  \addplot[rl text,rl line,forget plot] coordinates {(0,50.3) (50,51.5) (100,51.41) (150,54.2) (200,55.75)};
  \addplot[rl mm,rl line,forget plot] coordinates {(0,60.31) (50,61.14) (100,61.23) (150,63.19) (200,65.6)};
  \addplot[rl prod,rl line,forget plot] coordinates {(0,61.07) (50,62.54) (100,62.48) (150,62.72) (200,61.83)};
}
\newcommand{\RLBenchIFEval}{%
  \addplot[rl text,rl line,forget plot] coordinates {(0,71.16) (50,75.05) (100,75.23) (150,81.33) (200,82.62)};
  \addplot[rl mm,rl line,forget plot] coordinates {(0,75.97) (50,73.38) (100,79.11) (150,80.96) (200,82.26)};
  \addplot[rl prod,rl line,forget plot] coordinates {(0,75.05) (50,76.16) (100,75.05) (150,78.56) (200,78.56)};
}
\newcommand{\RLBenchMultiIF}{%
  \addplot[rl text,rl line,forget plot] coordinates {(0,69.34) (50,70.38) (100,73.74) (150,78.07) (200,80)};
  \addplot[rl mm,rl line,forget plot] coordinates {(0,70.03) (50,71.65) (100,74.69) (150,76.29) (200,78.27)};
  \addplot[rl prod,rl line,forget plot] coordinates {(0,69.32) (50,71.56) (100,71.83) (150,74.85) (200,76.12)};
}
\newcommand{\RLBenchIFBench}{%
  \addplot[rl text,rl line,forget plot] coordinates {(0,18) (50,20) (100,22) (150,24.67) (200,30.33)};
  \addplot[rl mm,rl line,forget plot] coordinates {(0,15.33) (50,16.67) (100,22.67) (150,23.33) (200,28.33)};
  \addplot[rl prod,rl line,forget plot] coordinates {(0,20.67) (50,17) (100,19.33) (150,19) (200,19)};
}


==> figs/post_training/rl_ablation_training_data.tex <==
\newcommand{\RLTrainRewardMath}{%
  \addplot[rl text,rl curve,forget plot] coordinates {(4,0.1377) (6,0.1426) (8,0.1442) (10,0.1467) (12,0.1498) (14,0.1563) (16,0.1568) (18,0.1617) (20,0.1668) (22,0.1732) (24,0.173) (26,0.1772) (28,0.1775) (30,0.1727) (32,0.1713) (34,0.1697) (36,0.1809) (38,0.1762) (40,0.1781) (42,0.1807) (44,0.1881) (46,0.1834) (48,0.1859) (50,0.1895) (52,0.1852) (54,0.1955) (56,0.1865) (58,0.1861) (60,0.1895) (62,0.192) (64,0.1811) (66,0.193) (68,0.2113) (70,0.2225) (72,0.2203) (74,0.227) (76,0.2307) (78,0.2289) (80,0.2281) (82,0.2402) (84,0.2416) (86,0.2463) (88,0.2387) (90,0.2387) (92,0.2301) (94,0.2311) (96,0.2363) (98,0.2313) (100,0.2301) (102,0.2363) (104,0.2396) (106,0.2381) (108,0.2439) (110,0.2426) (112,0.2512) (114,0.2453) (116,0.2428) (118,0.2607) (120,0.2711) (122,0.2721) (124,0.2703) (126,0.2678) (128,0.267) (130,0.2639) (132,0.2553) (134,0.2672) (136,0.2695) (138,0.2742) (140,0.2762) (142,0.2752) (144,0.2615) (146,0.2697) (148,0.2592) (150,0.2508) (152,0.2703) (154,0.2822) (156,0.2863) (158,0.2787) (160,0.2922) (162,0.274) (164,0.273) (166,0.2609) (168,0.2693) (170,0.2676) (172,0.277) (174,0.2816) (176,0.2867) (178,0.2883) (180,0.2828) (182,0.2932) (184,0.2953) (186,0.2996) (188,0.2975) (190,0.2943) (192,0.2898) (194,0.2887) (196,0.2844) (198,0.292) (200,0.2859)};
  \addplot[rl text,rl marks] coordinates {(50,0.1895) (100,0.2301) (150,0.2508) (200,0.2859)};
  \addplot[rl mm,rl curve,forget plot] coordinates {(4,0.1914) (6,0.1904) (8,0.1921) (10,0.188) (12,0.1938) (14,0.1967) (16,0.1986) (18,0.2029) (20,0.209) (22,0.2131) (24,0.2186) (26,0.2191) (28,0.2191) (30,0.227) (32,0.2258) (34,0.2248) (36,0.2367) (38,0.2398) (40,0.2408) (42,0.2486) (44,0.2527) (46,0.25) (48,0.2447) (50,0.2432) (52,0.2412) (54,0.25) (56,0.2488) (58,0.2469) (60,0.2553) (62,0.2547) (64,0.2449) (66,0.2555) (68,0.2807) (70,0.2828) (72,0.2881) (74,0.2947) (76,0.2988) (78,0.3051) (80,0.301) (82,0.3008) (84,0.3064) (86,0.3102) (88,0.2906) (90,0.2988) (92,0.3008) (94,0.2918) (96,0.2967) (98,0.2949) (100,0.3037) (102,0.3086) (104,0.3195) (106,0.3137) (108,0.3195) (110,0.3068) (112,0.3158) (114,0.3088) (116,0.3107) (118,0.3291) (120,0.3445) (122,0.3404) (124,0.35) (126,0.3373) (128,0.3381) (130,0.3352) (132,0.3289) (134,0.3352) (136,0.3498) (138,0.351) (140,0.3479) (142,0.3479) (144,0.3365) (146,0.3359) (148,0.3264) (150,0.3199) (152,0.3396) (154,0.3434) (156,0.3539) (158,0.3441) (160,0.3615) (162,0.3412) (164,0.3434) (166,0.3297) (168,0.3434) (170,0.3346) (172,0.3451) (174,0.3479) (176,0.3566) (178,0.3615) (180,0.3594) (182,0.367) (184,0.3809) (186,0.3816) (188,0.3828) (190,0.3822) (192,0.3734) (194,0.3729) (196,0.3764) (198,0.3736) (200,0.3695)};
  \addplot[rl mm,rl marks] coordinates {(50,0.2432) (100,0.3037) (150,0.3199) (200,0.3695)};
  \addplot[rl prod,rl curve,forget plot] coordinates {(4,0.3496) (6,0.3608) (8,0.3646) (10,0.3677) (12,0.3678) (14,0.3813) (16,0.3814) (18,0.3893) (20,0.3957) (22,0.4023) (24,0.4016) (26,0.4014) (28,0.3982) (30,0.3805) (32,0.3707) (34,0.3631) (36,0.376) (38,0.3732) (40,0.3842) (42,0.4023) (44,0.4006) (46,0.3902) (48,0.3918) (50,0.3922) (52,0.374) (54,0.3943) (56,0.3826) (58,0.3656) (60,0.3676) (62,0.3732) (64,0.3578) (66,0.376) (68,0.4035) (70,0.398) (72,0.4121) (74,0.4113) (76,0.4195) (78,0.4172) (80,0.4205) (82,0.4154) (84,0.4158) (86,0.407) (88,0.3924) (90,0.402) (92,0.3887) (94,0.3967) (96,0.3861) (98,0.3818) (100,0.3811) (102,0.3824) (104,0.3807) (106,0.3816) (108,0.3816) (110,0.3697) (112,0.3883) (114,0.3713) (116,0.3875) (118,0.4105) (120,0.4193) (122,0.4098) (124,0.4252) (126,0.41) (128,0.4062) (130,0.4107) (132,0.4121) (134,0.4135) (136,0.4158) (138,0.427) (140,0.4352) (142,0.4178) (144,0.4143) (146,0.4184) (148,0.3975) (150,0.3834) (152,0.4141) (154,0.4219) (156,0.4186) (158,0.4086) (160,0.4189) (162,0.4043) (164,0.4012) (166,0.407) (168,0.4164) (170,0.4211) (172,0.4232) (174,0.4115) (176,0.4188) (178,0.4334) (180,0.4186) (182,0.4334) (184,0.4512) (186,0.4547) (188,0.4445) (190,0.4428) (192,0.4334) (194,0.4275) (196,0.4264) (198,0.427) (200,0.4252)};
  \addplot[rl prod,rl marks] coordinates {(50,0.3922) (100,0.3811) (150,0.3834) (200,0.4252)};
}
\newcommand{\RLTrainLengthMath}{%
  \addplot[rl text,rl curve,forget plot] coordinates {(4,10.18) (6,10.05) (8,10) (10,9.993) (12,9.936) (14,9.771) (16,9.785) (18,9.77) (20,9.737) (22,9.702) (24,9.749) (26,9.709) (28,9.693) (30,9.703) (32,9.685) (34,9.792) (36,9.741) (38,9.742) (40,9.785) (42,9.758) (44,9.576) (46,9.61) (48,9.63) (50,9.608) (52,9.741) (54,9.702) (56,9.707) (58,9.745) (60,9.747) (62,9.669) (64,9.775) (66,9.686) (68,9.475) (70,9.282) (72,9.271) (74,9.244) (76,9.305) (78,9.349) (80,9.442) (82,9.451) (84,9.469) (86,9.439) (88,9.579) (90,9.545) (92,9.617) (94,9.662) (96,9.588) (98,9.609) (100,9.63) (102,9.517) (104,9.528) (106,9.6) (108,9.602) (110,9.695) (112,9.622) (114,9.588) (116,9.628) (118,9.491) (120,9.349) (122,9.381) (124,9.535) (126,9.522) (128,9.541) (130,9.618) (132,9.725) (134,9.607) (136,9.592) (138,9.528) (140,9.543) (142,9.619) (144,9.594) (146,9.504) (148,9.657) (150,9.639) (152,9.453) (154,9.488) (156,9.527) (158,9.576) (160,9.524) (162,9.684) (164,9.617) (166,9.742) (168,9.695) (170,9.699) (172,9.666) (174,9.603) (176,9.478) (178,9.437) (180,9.483) (182,9.374) (184,9.41) (186,9.346) (188,9.359) (190,9.421) (192,9.48) (194,9.446) (196,9.625) (198,9.603) (200,9.718)};
  \addplot[rl text,rl marks] coordinates {(50,9.608) (100,9.63) (150,9.639) (200,9.718)};
  \addplot[rl mm,rl curve,forget plot] coordinates {(4,9.972) (6,10.03) (8,10.11) (10,10.05) (12,9.998) (14,9.989) (16,9.961) (18,9.938) (20,9.924) (22,9.911) (24,9.83) (26,9.881) (28,9.858) (30,9.825) (32,9.807) (34,9.889) (36,9.729) (38,9.706) (40,9.726) (42,9.673) (44,9.596) (46,9.689) (48,9.655) (50,9.705) (52,9.867) (54,9.878) (56,9.901) (58,9.989) (60,10.02) (62,9.991) (64,10.08) (66,10.03) (68,9.837) (70,9.72) (72,9.646) (74,9.589) (76,9.59) (78,9.652) (80,9.708) (82,9.739) (84,9.708) (86,9.648) (88,9.774) (90,9.741) (92,9.745) (94,9.856) (96,9.833) (98,9.799) (100,9.803) (102,9.71) (104,9.543) (106,9.629) (108,9.632) (110,9.718) (112,9.684) (114,9.775) (116,9.759) (118,9.633) (120,9.442) (122,9.495) (124,9.547) (126,9.613) (128,9.6) (130,9.716) (132,9.781) (134,9.688) (136,9.594) (138,9.554) (140,9.564) (142,9.559) (144,9.585) (146,9.551) (148,9.679) (150,9.687) (152,9.539) (154,9.495) (156,9.439) (158,9.503) (160,9.4) (162,9.517) (164,9.505) (166,9.636) (168,9.532) (170,9.547) (172,9.498) (174,9.501) (176,9.37) (178,9.291) (180,9.361) (182,9.303) (184,9.244) (186,9.279) (188,9.318) (190,9.275) (192,9.375) (194,9.284) (196,9.312) (198,9.292) (200,9.346)};
  \addplot[rl mm,rl marks] coordinates {(50,9.705) (100,9.803) (150,9.687) (200,9.346)};
  \addplot[rl prod,rl curve,forget plot] coordinates {(4,9.528) (6,9.364) (8,9.288) (10,9.288) (12,9.331) (14,9.258) (16,9.343) (18,9.345) (20,9.27) (22,9.171) (24,9.104) (26,9.064) (28,9.112) (30,9.231) (32,9.288) (34,9.447) (36,9.35) (38,9.326) (40,9.325) (42,9.166) (44,9.048) (46,9.095) (48,9.087) (50,9.047) (52,9.302) (54,9.164) (56,9.24) (58,9.36) (60,9.377) (62,9.32) (64,9.485) (66,9.382) (68,9.104) (70,9.078) (72,8.867) (74,8.885) (76,8.84) (78,8.967) (80,9.001) (82,9.066) (84,9.035) (86,9.07) (88,9.16) (90,9.057) (92,9.197) (94,9.157) (96,9.235) (98,9.267) (100,9.234) (102,9.137) (104,9.147) (106,9.158) (108,9.167) (110,9.305) (112,9.17) (114,9.233) (116,9.101) (118,8.915) (120,8.838) (122,8.968) (124,8.959) (126,9.039) (128,8.982) (130,9.021) (132,8.99) (134,8.939) (136,8.906) (138,8.94) (140,8.796) (142,8.967) (144,8.954) (146,8.911) (148,9.023) (150,9.139) (152,8.827) (154,8.74) (156,8.786) (158,8.841) (160,8.769) (162,8.909) (164,8.907) (166,8.978) (168,8.892) (170,8.85) (172,8.894) (174,9.002) (176,8.857) (178,8.763) (180,8.942) (182,8.757) (184,8.705) (186,8.659) (188,8.75) (190,8.664) (192,8.785) (194,8.769) (196,8.823) (198,8.836) (200,8.897)};
  \addplot[rl prod,rl marks] coordinates {(50,9.047) (100,9.234) (150,9.139) (200,8.897)};
}
\newcommand{\RLTrainRewardReasoning}{%
  \addplot[rl text,rl curve,forget plot] coordinates {(4,0.1387) (6,0.1475) (8,0.1836) (10,0.1941) (12,0.21) (14,0.2158) (16,0.2188) (18,0.2098) (20,0.2002) (22,0.1887) (24,0.1973) (26,0.1957) (28,0.2006) (30,0.2113) (32,0.2074) (34,0.2197) (36,0.2316) (38,0.2283) (40,0.2324) (42,0.2457) (44,0.2447) (46,0.2355) (48,0.232) (50,0.2383) (52,0.2283) (54,0.2283) (56,0.2314) (58,0.2332) (60,0.2246) (62,0.2125) (64,0.2004) (66,0.207) (68,0.2244) (70,0.2238) (72,0.2531) (74,0.2568) (76,0.2559) (78,0.2549) (80,0.2516) (82,0.2336) (84,0.2404) (86,0.2504) (88,0.2469) (90,0.2463) (92,0.2502) (94,0.243) (96,0.2498) (98,0.24) (100,0.2457) (102,0.25) (104,0.2686) (106,0.2492) (108,0.2498) (110,0.2555) (112,0.2564) (114,0.2461) (116,0.2568) (118,0.2752) (120,0.2877) (122,0.2873) (124,0.2943) (126,0.2916) (128,0.2727) (130,0.2559) (132,0.2682) (134,0.2611) (136,0.258) (138,0.2625) (140,0.2691) (142,0.2543) (144,0.2621) (146,0.2656) (148,0.2762) (150,0.2861) (152,0.2859) (154,0.2807) (156,0.2676) (158,0.2852) (160,0.2717) (162,0.2715) (164,0.2756) (166,0.2881) (168,0.2652) (170,0.2652) (172,0.2828) (174,0.2764) (176,0.2748) (178,0.285) (180,0.2953) (182,0.2916) (184,0.2793) (186,0.285) (188,0.2777) (190,0.2693) (192,0.265) (194,0.2779) (196,0.285) (198,0.2766) (200,0.2799)};
  \addplot[rl text,rl marks] coordinates {(50,0.2383) (100,0.2457) (150,0.2861) (200,0.2799)};
  \addplot[rl mm,rl curve,forget plot] coordinates {(4,0.2949) (6,0.2642) (8,0.2988) (10,0.2981) (12,0.2955) (14,0.2848) (16,0.2949) (18,0.2738) (20,0.258) (22,0.26) (24,0.2645) (26,0.26) (28,0.2596) (30,0.2762) (32,0.2736) (34,0.2875) (36,0.2895) (38,0.299) (40,0.2984) (42,0.2943) (44,0.2984) (46,0.3029) (48,0.2879) (50,0.282) (52,0.3) (54,0.2885) (56,0.2885) (58,0.2986) (60,0.31) (62,0.2867) (64,0.2814) (66,0.274) (68,0.282) (70,0.2727) (72,0.2955) (74,0.3086) (76,0.3207) (78,0.3029) (80,0.3129) (82,0.2908) (84,0.2848) (86,0.2896) (88,0.3) (90,0.3057) (92,0.3254) (94,0.3203) (96,0.3094) (98,0.3324) (100,0.3186) (102,0.3156) (104,0.3197) (106,0.3297) (108,0.3088) (110,0.3164) (112,0.3094) (114,0.3143) (116,0.3006) (118,0.3107) (120,0.3104) (122,0.3287) (124,0.3346) (126,0.3455) (128,0.3387) (130,0.3359) (132,0.3203) (134,0.3086) (136,0.3162) (138,0.3125) (140,0.3031) (142,0.307) (144,0.3146) (146,0.3055) (148,0.3143) (150,0.3344) (152,0.3402) (154,0.3518) (156,0.3463) (158,0.3467) (160,0.3301) (162,0.3373) (164,0.3348) (166,0.3412) (168,0.3324) (170,0.3424) (172,0.3217) (174,0.3207) (176,0.3258) (178,0.3475) (180,0.3453) (182,0.3586) (184,0.3562) (186,0.3564) (188,0.3385) (190,0.3385) (192,0.3342) (194,0.3338) (196,0.3332) (198,0.3285) (200,0.3445)};
  \addplot[rl mm,rl marks] coordinates {(50,0.282) (100,0.3186) (150,0.3344) (200,0.3445)};
  \addplot[rl prod,rl curve,forget plot] coordinates {(4,0.3545) (6,0.3291) (8,0.3408) (10,0.3516) (12,0.3551) (14,0.3379) (16,0.3469) (18,0.3273) (20,0.3084) (22,0.3072) (24,0.3117) (26,0.2945) (28,0.3113) (30,0.3293) (32,0.3098) (34,0.3332) (36,0.3357) (38,0.3352) (40,0.3262) (42,0.3324) (44,0.3312) (46,0.3357) (48,0.3176) (50,0.3328) (52,0.3342) (54,0.325) (56,0.3307) (58,0.3424) (60,0.3289) (62,0.3215) (64,0.3068) (66,0.3018) (68,0.3148) (70,0.3186) (72,0.3408) (74,0.3473) (76,0.3502) (78,0.3375) (80,0.3281) (82,0.3068) (84,0.3119) (86,0.3217) (88,0.3242) (90,0.3332) (92,0.3609) (94,0.352) (96,0.3482) (98,0.3541) (100,0.3475) (102,0.333) (104,0.3371) (106,0.333) (108,0.3299) (110,0.3309) (112,0.3266) (114,0.3287) (116,0.3359) (118,0.3293) (120,0.352) (122,0.3695) (124,0.3672) (126,0.3633) (128,0.3652) (130,0.3307) (132,0.3252) (134,0.3355) (136,0.3326) (138,0.3303) (140,0.3461) (142,0.3352) (144,0.3264) (146,0.3377) (148,0.3512) (150,0.3543) (152,0.3613) (154,0.3578) (156,0.343) (158,0.3299) (160,0.3371) (162,0.3289) (164,0.3311) (166,0.3334) (168,0.3328) (170,0.326) (172,0.3379) (174,0.3568) (176,0.3625) (178,0.3736) (180,0.3756) (182,0.3746) (184,0.358) (186,0.3521) (188,0.3576) (190,0.3553) (192,0.3604) (194,0.3602) (196,0.3564) (198,0.3609) (200,0.36)};
  \addplot[rl prod,rl marks] coordinates {(50,0.3328) (100,0.3475) (150,0.3543) (200,0.36)};
}
\newcommand{\RLTrainLengthReasoning}{%
  \addplot[rl text,rl curve,forget plot] coordinates {(4,3.407) (6,3.177) (8,2.502) (10,2.704) (12,2.482) (14,2.373) (16,2.373) (18,2.63) (20,2.498) (22,2.819) (24,2.868) (26,2.781) (28,2.804) (30,2.931) (32,2.866) (34,2.67) (36,2.839) (38,2.98) (40,2.818) (42,2.74) (44,2.908) (46,2.969) (48,3.185) (50,3.35) (52,3.467) (54,3.596) (56,3.526) (58,3.526) (60,3.522) (62,3.756) (64,3.827) (66,3.881) (68,3.63) (70,3.781) (72,3.638) (74,3.641) (76,3.722) (78,3.864) (80,3.812) (82,3.885) (84,3.853) (86,3.713) (88,3.851) (90,3.918) (92,3.783) (94,3.913) (96,4.257) (98,4.121) (100,3.967) (102,4.334) (104,4.095) (106,3.935) (108,4.178) (110,4.418) (112,4.233) (114,4.299) (116,4.287) (118,4.131) (120,4.162) (122,4.358) (124,4.617) (126,4.817) (128,5.21) (130,5.357) (132,5.03) (134,5.117) (136,5.355) (138,4.996) (140,4.866) (142,5.198) (144,4.98) (146,4.711) (148,4.718) (150,4.724) (152,4.853) (154,5.128) (156,5.367) (158,5.224) (160,5.277) (162,5.304) (164,5.254) (166,4.985) (168,5.407) (170,5.618) (172,5.477) (174,5.443) (176,5.415) (178,5.396) (180,5.268) (182,5.182) (184,5.381) (186,5.553) (188,5.425) (190,5.518) (192,5.671) (194,5.579) (196,5.433) (198,5.663) (200,5.456)};
  \addplot[rl text,rl marks] coordinates {(50,3.35) (100,3.967) (150,4.724) (200,5.456)};
  \addplot[rl mm,rl curve,forget plot] coordinates {(4,4.633) (6,5.266) (8,5.149) (10,5.269) (12,5.401) (14,5.58) (16,5.589) (18,5.669) (20,5.841) (22,5.849) (24,5.889) (26,5.884) (28,6.037) (30,5.93) (32,5.846) (34,5.686) (36,5.739) (38,5.684) (40,5.704) (42,5.899) (44,5.883) (46,5.951) (48,6.183) (50,6.288) (52,6.018) (54,6.229) (56,6.23) (58,6.014) (60,5.966) (62,6.24) (64,6.325) (66,6.264) (68,6.258) (70,6.247) (72,6) (74,5.95) (76,5.974) (78,6.079) (80,5.971) (82,6.264) (84,6.22) (86,6.081) (88,6.153) (90,6.158) (92,5.977) (94,6.094) (96,6.268) (98,6.039) (100,6.167) (102,6.283) (104,6.286) (106,6.166) (108,6.333) (110,6.284) (112,6.211) (114,6.072) (116,6.097) (118,6.051) (120,5.969) (122,6.006) (124,6.044) (126,6.132) (128,6.232) (130,6.43) (132,6.496) (134,6.58) (136,6.43) (138,6.401) (140,6.485) (142,6.445) (144,6.372) (146,6.493) (148,6.408) (150,6.129) (152,5.976) (154,5.969) (156,6.081) (158,6.216) (160,6.383) (162,6.423) (164,6.43) (166,6.378) (168,6.345) (170,6.256) (172,6.449) (174,6.455) (176,6.472) (178,6.333) (180,6.397) (182,6.271) (184,6.367) (186,6.29) (188,6.387) (190,6.443) (192,6.45) (194,6.48) (196,6.538) (198,6.593) (200,6.437)};
  \addplot[rl mm,rl marks] coordinates {(50,6.288) (100,6.167) (150,6.129) (200,6.437)};
  \addplot[rl prod,rl curve,forget plot] coordinates {(4,6.24) (6,6.484) (8,6.572) (10,6.674) (12,6.761) (14,7.085) (16,7.136) (18,7.381) (20,7.411) (22,7.413) (24,7.317) (26,7.416) (28,7.11) (30,7.044) (32,7.078) (34,6.814) (36,6.814) (38,6.868) (40,6.915) (42,6.925) (44,6.903) (46,6.92) (48,7.221) (50,7.08) (52,6.962) (54,7.206) (56,7.207) (58,6.957) (60,7.135) (62,7.383) (64,7.38) (66,7.357) (68,7.329) (70,7.301) (72,6.92) (74,6.969) (76,7.03) (78,7.032) (80,7.08) (82,7.357) (84,7.252) (86,7.005) (88,6.987) (90,6.948) (92,6.669) (94,6.882) (96,7.004) (98,7.098) (100,7.153) (102,7.348) (104,7.23) (106,7.291) (108,7.32) (110,7.221) (112,7.268) (114,7.11) (116,7.001) (118,6.871) (120,6.81) (122,6.632) (124,6.807) (126,6.909) (128,7.063) (130,7.302) (132,7.422) (134,7.225) (136,7.195) (138,7.233) (140,7.033) (142,7.02) (144,7.094) (146,6.975) (148,6.722) (150,6.648) (152,6.631) (154,6.732) (156,7.009) (158,7.159) (160,7.065) (162,7.137) (164,7.108) (166,6.897) (168,6.934) (170,7.184) (172,7.019) (174,6.917) (176,6.887) (178,6.744) (180,6.715) (182,6.888) (184,6.925) (186,7.134) (188,7.026) (190,7.056) (192,6.955) (194,7.052) (196,6.939) (198,6.98) (200,6.9)};
  \addplot[rl prod,rl marks] coordinates {(50,7.08) (100,7.153) (150,6.648) (200,6.9)};
}
\newcommand{\RLTrainRewardIF}{%
  \addplot[rl text,rl curve,forget plot] coordinates {(4,0.2832) (6,0.3027) (8,0.3099) (10,0.311) (12,0.315) (14,0.316) (16,0.327) (18,0.3324) (20,0.3428) (22,0.3484) (24,0.3613) (26,0.3576) (28,0.358) (30,0.3598) (32,0.3588) (34,0.3639) (36,0.3742) (38,0.374) (40,0.3818) (42,0.3768) (44,0.3693) (46,0.3703) (48,0.3598) (50,0.3594) (52,0.367) (54,0.376) (56,0.3676) (58,0.3756) (60,0.367) (62,0.3629) (64,0.3609) (66,0.368) (68,0.3838) (70,0.402) (72,0.4143) (74,0.4207) (76,0.4227) (78,0.4238) (80,0.4139) (82,0.4049) (84,0.3865) (86,0.3879) (88,0.384) (90,0.3918) (92,0.4061) (94,0.4293) (96,0.427) (98,0.4328) (100,0.4268) (102,0.4305) (104,0.4348) (106,0.4453) (108,0.4568) (110,0.4687) (112,0.4736) (114,0.4729) (116,0.4777) (118,0.476) (120,0.4816) (122,0.4834) (124,0.4867) (126,0.4832) (128,0.4814) (130,0.4785) (132,0.4766) (134,0.4822) (136,0.4805) (138,0.4926) (140,0.4979) (142,0.5002) (144,0.4959) (146,0.5049) (148,0.508) (150,0.5008) (152,0.5025) (154,0.5184) (156,0.5115) (158,0.4969) (160,0.4957) (162,0.5041) (164,0.5133) (166,0.5133) (168,0.5176) (170,0.5232) (172,0.5164) (174,0.491) (176,0.5055) (178,0.5215) (180,0.5168) (182,0.5094) (184,0.5172) (186,0.5008) (188,0.4855) (190,0.4984) (192,0.5125) (194,0.5057) (196,0.515) (198,0.5176) (200,0.5125)};
  \addplot[rl text,rl marks] coordinates {(50,0.3594) (100,0.4268) (150,0.5008) (200,0.5125)};
  \addplot[rl mm,rl curve,forget plot] coordinates {(4,0.3027) (6,0.3286) (8,0.3333) (10,0.3374) (12,0.3398) (14,0.3424) (16,0.3473) (18,0.3535) (20,0.3592) (22,0.3637) (24,0.3766) (26,0.3738) (28,0.3678) (30,0.3693) (32,0.3705) (34,0.3754) (36,0.3898) (38,0.3928) (40,0.3937) (42,0.3928) (44,0.3812) (46,0.3748) (48,0.3637) (50,0.3742) (52,0.3795) (54,0.3889) (56,0.3801) (58,0.3908) (60,0.3758) (62,0.3658) (64,0.3633) (66,0.3785) (68,0.3916) (70,0.4084) (72,0.4197) (74,0.4283) (76,0.4207) (78,0.4209) (80,0.4123) (82,0.4049) (84,0.3824) (86,0.3846) (88,0.3859) (90,0.3893) (92,0.4039) (94,0.4285) (96,0.4354) (98,0.4387) (100,0.4355) (102,0.4406) (104,0.4398) (106,0.4406) (108,0.448) (110,0.4564) (112,0.4611) (114,0.466) (116,0.4682) (118,0.4676) (120,0.4693) (122,0.4588) (124,0.4561) (126,0.4564) (128,0.4521) (130,0.4576) (132,0.4607) (134,0.4717) (136,0.4613) (138,0.4793) (140,0.484) (142,0.4826) (144,0.4811) (146,0.4926) (148,0.49) (150,0.4781) (152,0.4934) (154,0.501) (156,0.5023) (158,0.4875) (160,0.4912) (162,0.4936) (164,0.4996) (166,0.5006) (168,0.5068) (170,0.5062) (172,0.5004) (174,0.4893) (176,0.5059) (178,0.5156) (180,0.5182) (182,0.5066) (184,0.5002) (186,0.4805) (188,0.4764) (190,0.4816) (192,0.5004) (194,0.4914) (196,0.502) (198,0.5023) (200,0.4973)};
  \addplot[rl mm,rl marks] coordinates {(50,0.3742) (100,0.4355) (150,0.4781) (200,0.4973)};
  \addplot[rl prod,rl curve,forget plot] coordinates {(4,0.2764) (6,0.3071) (8,0.3092) (10,0.3157) (12,0.3188) (14,0.3207) (16,0.3236) (18,0.3303) (20,0.3314) (22,0.3369) (24,0.3537) (26,0.3488) (28,0.3443) (30,0.3516) (32,0.3482) (34,0.3477) (36,0.3607) (38,0.3654) (40,0.3689) (42,0.366) (44,0.3574) (46,0.3547) (48,0.3477) (50,0.3484) (52,0.3527) (54,0.3637) (56,0.3574) (58,0.3633) (60,0.349) (62,0.3473) (64,0.3398) (66,0.3463) (68,0.3527) (70,0.3664) (72,0.374) (74,0.3789) (76,0.3764) (78,0.3748) (80,0.368) (82,0.3609) (84,0.3486) (86,0.3506) (88,0.3484) (90,0.3523) (92,0.3646) (94,0.3785) (96,0.3836) (98,0.393) (100,0.3871) (102,0.3877) (104,0.3926) (106,0.4008) (108,0.4033) (110,0.4193) (112,0.4197) (114,0.4236) (116,0.4199) (118,0.4244) (120,0.4191) (122,0.4143) (124,0.4088) (126,0.4035) (128,0.3932) (130,0.3961) (132,0.4029) (134,0.4107) (136,0.4055) (138,0.4189) (140,0.425) (142,0.4242) (144,0.423) (146,0.4334) (148,0.4375) (150,0.4318) (152,0.4385) (154,0.4455) (156,0.4469) (158,0.4414) (160,0.4385) (162,0.4422) (164,0.451) (166,0.4436) (168,0.4441) (170,0.4492) (172,0.4449) (174,0.4254) (176,0.4432) (178,0.4494) (180,0.4477) (182,0.4395) (184,0.4508) (186,0.4262) (188,0.4199) (190,0.426) (192,0.4426) (194,0.4311) (196,0.4459) (198,0.4437) (200,0.4342)};
  \addplot[rl prod,rl marks] coordinates {(50,0.3484) (100,0.3871) (150,0.4318) (200,0.4342)};
}
\newcommand{\RLTrainLengthIF}{%
  \addplot[rl text,rl curve,forget plot] coordinates {(4,0.3927) (6,0.3837) (8,0.4021) (10,0.4001) (12,0.3968) (14,0.4087) (16,0.409) (18,0.4002) (20,0.3928) (22,0.3889) (24,0.3816) (26,0.392) (28,0.3876) (30,0.3749) (32,0.3759) (34,0.3638) (36,0.3613) (38,0.3595) (40,0.3731) (42,0.3792) (44,0.3747) (46,0.3602) (48,0.3565) (50,0.3496) (52,0.3341) (54,0.347) (56,0.3496) (58,0.337) (60,0.3359) (62,0.3463) (64,0.3222) (66,0.3225) (68,0.3318) (70,0.3289) (72,0.3182) (74,0.325) (76,0.3274) (78,0.3257) (80,0.3265) (82,0.3256) (84,0.3342) (86,0.3237) (88,0.3302) (90,0.3342) (92,0.3364) (94,0.327) (96,0.315) (98,0.3063) (100,0.2958) (102,0.2891) (104,0.2776) (106,0.2803) (108,0.269) (110,0.2703) (112,0.2647) (114,0.2721) (116,0.2692) (118,0.2657) (120,0.2553) (122,0.2553) (124,0.2471) (126,0.2419) (128,0.2451) (130,0.2428) (132,0.2287) (134,0.2248) (136,0.2222) (138,0.2109) (140,0.218) (142,0.2214) (144,0.214) (146,0.2116) (148,0.2073) (150,0.186) (152,0.1937) (154,0.1899) (156,0.1882) (158,0.1866) (160,0.1948) (162,0.1809) (164,0.1875) (166,0.1892) (168,0.1961) (170,0.1922) (172,0.1931) (174,0.186) (176,0.1791) (178,0.1743) (180,0.1688) (182,0.1719) (184,0.1693) (186,0.1679) (188,0.1618) (190,0.169) (192,0.1576) (194,0.1563) (196,0.1519) (198,0.1579) (200,0.1514)};
  \addplot[rl text,rl marks] coordinates {(50,0.3496) (100,0.2958) (150,0.186) (200,0.1514)};
  \addplot[rl mm,rl curve,forget plot] coordinates {(4,0.3623) (6,0.3521) (8,0.3644) (10,0.3614) (12,0.361) (14,0.3667) (16,0.3682) (18,0.3673) (20,0.3637) (22,0.3615) (24,0.3562) (26,0.367) (28,0.3655) (30,0.3601) (32,0.3722) (34,0.3696) (36,0.3677) (38,0.3656) (40,0.3792) (42,0.3745) (44,0.3718) (46,0.3595) (48,0.3562) (50,0.3471) (52,0.3428) (54,0.3536) (56,0.3552) (58,0.3417) (60,0.3448) (62,0.3554) (64,0.3335) (66,0.3325) (68,0.344) (70,0.3412) (72,0.3255) (74,0.3347) (76,0.3517) (78,0.3529) (80,0.3566) (82,0.3563) (84,0.3623) (86,0.3477) (88,0.3546) (90,0.362) (92,0.3558) (94,0.3488) (96,0.3334) (98,0.3221) (100,0.3145) (102,0.3199) (104,0.3142) (106,0.3194) (108,0.3156) (110,0.3133) (112,0.3072) (114,0.315) (116,0.3162) (118,0.3144) (120,0.309) (122,0.3142) (124,0.31) (126,0.3065) (128,0.2938) (130,0.2834) (132,0.264) (134,0.2548) (136,0.255) (138,0.2574) (140,0.2633) (142,0.2746) (144,0.2687) (146,0.2663) (148,0.2655) (150,0.2478) (152,0.2575) (154,0.2632) (156,0.2597) (158,0.2529) (160,0.265) (162,0.2359) (164,0.2281) (166,0.2357) (168,0.2377) (170,0.2312) (172,0.239) (174,0.2321) (176,0.2162) (178,0.2103) (180,0.2035) (182,0.201) (184,0.2008) (186,0.1954) (188,0.1895) (190,0.1906) (192,0.1834) (194,0.1778) (196,0.1721) (198,0.1755) (200,0.1702)};
  \addplot[rl mm,rl marks] coordinates {(50,0.3471) (100,0.3145) (150,0.2478) (200,0.1702)};
  \addplot[rl prod,rl curve,forget plot] coordinates {(4,0.375) (6,0.3552) (8,0.3712) (10,0.3689) (12,0.369) (14,0.3783) (16,0.3838) (18,0.386) (20,0.3878) (22,0.3873) (24,0.3764) (26,0.3952) (28,0.3943) (30,0.3838) (32,0.3883) (34,0.3911) (36,0.3851) (38,0.3791) (40,0.398) (42,0.4062) (44,0.4004) (46,0.3843) (48,0.3828) (50,0.3717) (52,0.3564) (54,0.3681) (56,0.3779) (58,0.3662) (60,0.3695) (62,0.38) (64,0.3645) (66,0.3657) (68,0.3819) (70,0.3796) (72,0.3727) (74,0.379) (76,0.3757) (78,0.376) (80,0.3806) (82,0.3839) (84,0.3907) (86,0.3912) (88,0.3879) (90,0.3908) (92,0.3871) (94,0.3784) (96,0.3635) (98,0.356) (100,0.3623) (102,0.3554) (104,0.3564) (106,0.3619) (108,0.3604) (110,0.3454) (112,0.3473) (114,0.3508) (116,0.3522) (118,0.355) (120,0.3602) (122,0.364) (124,0.3658) (126,0.36) (128,0.3575) (130,0.3434) (132,0.3325) (134,0.3299) (136,0.3432) (138,0.3301) (140,0.3348) (142,0.3479) (144,0.3345) (146,0.3252) (148,0.3346) (150,0.3182) (152,0.3208) (154,0.3289) (156,0.3288) (158,0.3273) (160,0.3411) (162,0.3262) (164,0.3179) (166,0.3176) (168,0.3155) (170,0.3067) (172,0.3018) (174,0.302) (176,0.2947) (178,0.2944) (180,0.289) (182,0.2979) (184,0.2809) (186,0.2822) (188,0.2756) (190,0.2794) (192,0.2592) (194,0.265) (196,0.2477) (198,0.254) (200,0.2556)};
  \addplot[rl prod,rl marks] coordinates {(50,0.3717) (100,0.3623) (150,0.3182) (200,0.2556)};
}


==> figs/post_training/sft_ablation_questions_data.tex <==
\newcommand{\SFTPanelA}{%
  \addplot[sft mean] coordinates {(0,0.035352391674) (1,0.919385589927) (2,3.128665897632)};
  \addplot[sft seed] coordinates {(-0.130000,0.288160601844) (0.000000,-0.207751997511) (0.130000,0.025648570690) (0.870000,1.310165758817) (1.000000,0.901420038376) (1.130000,0.546570972586) (1.870000,2.709367642824) (2.000000,3.385563444208) (2.130000,3.291066605866)};
  \node[sft value,anchor=south] at (axis cs:0,0.518160601844) {$0.0$};
  \node[sft value,anchor=south] at (axis cs:1,1.540165758817) {$+0.9$};
  \node[sft value,anchor=south] at (axis cs:2,3.615563444208) {$+3.1$};
}
\newcommand{\SFTPanelB}{%
  \addplot[sft mean] coordinates {(0,3.824716137853) (1,0.230579424768)};
  \addplot[sft seed] coordinates {(-0.090000,3.828981676591) (0.000000,4.006087171948) (0.090000,3.639079565021) (0.910000,-0.441527040210) (1.000000,0.730581360529) (1.090000,0.402683953985)};
  \node[sft value,anchor=south] at (axis cs:0,4.236087171948) {$+3.8$};
  \node[sft value,anchor=south] at (axis cs:1,0.960581360529) {$+0.2$};
}
\newcommand{\SFTPanelC}{%
  \addplot[sft mean] coordinates {(0,-2.234130049123) (1,0.017832828243)};
  \addplot[sft seed] coordinates {(-0.090000,-2.624047394938) (0.000000,-1.565513687515) (0.090000,-2.512829064917) (0.910000,0.155804786964) (1.000000,0.242971665879) (1.090000,-0.345277968113)};
  \node[sft value,anchor=north] at (axis cs:0,-2.854047394938) {$-2.2$};
  \node[sft value,anchor=south] at (axis cs:1,0.472971665879) {$0.0$};
}

